STream3R: Scalable Sequential 3D Reconstruction with Causal Transformer

We present STream3R, a novel approach to 3D reconstruction that reformulates pointmap prediction as a decoder-only Transformer problem. Existing state-of-the-art methods for multi-view reconstruction either depend on expensive global optimization or rely on simplistic memory mechanisms that scale poorly with sequence length. In contrast, STream3R introduces an streaming framework that processes image sequences efficiently using causal attention, inspired by advances in modern language modeling. By learning geometric priors from large-scale 3D datasets, STream3R generalizes well to diverse and challenging scenarios, including dynamic scenes where traditional methods often fail. Extensive experiments show that our method consistently outperforms prior work across both static and dynamic scene benchmarks. Moreover, STream3R is inherently compatible with LLM-style training infrastructure, enabling efficient large-scale pretraining and fine-tuning for various downstream 3D tasks. Our results underscore the potential of causal Transformer models for online 3D perception, paving the way for real-time 3D understanding in streaming environments. More details can be found in our project page: https://nirvanalan.github.io/projects/stream3r.

==> sections/checklist.tex <==
\section*{NeurIPS Paper Checklist}
\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The abstract and introduction accurately reflect the paper's contributions and scope at the end of each section.

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Please find it at Sec.~\ref{sec:conclusion_discussion_limitation}.

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not include any theoretical result.


    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The experiments can be easily reproduced with the information provided in the implementation details section in Sec.~\ref{sec:experiment}.

\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We only use publicly available datasets and pre-processing code for training our models. The code will be open sourced upon acceptance.


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper has already included all the training and test details in the experiments section, and all the results can be reproduced with the provided information.
    
\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The proposed model is a deterministic model and does not have variations in the final results.


\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The experiments compute resources are included in the experiments section.
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper follow the NeurIPS Code of Ethics in every respect.


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The proposed method aims for 3D scene reconstruction and has the potential to serve as the  building blocks for many downstream applications, including embodied AI, scene understanding. Also, the proposed technology has the potential be used in military services.
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No LLMs, image generators, or scraped datasets are used in this paper.


\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All the creators of the original owners are properly mentioned and credited.


\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not release new assets.

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not include crowdsourcing research.


\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.


\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This core method development in this paper does not involve LLMs as any important, original, or non-standard components.

\end{enumerate}


==> sections/discussions.tex <==
\subsection{Limitations and future work}

Limitations:
The 3D shapes of the objects discussed in this paper can still be encoded with a single latent code.

% A similar observation is also found in~\cite{esser2024sd3}, where separate model parameters handle different modalities individually. 

Future work:
geometry side:
3D shapes with large variations such as human.
more complex, adopt local features to predict the geometry along with the global features.

texture side:
currently we only adopt a basic 2D hour-glass encoder to restoring the missing 3D information form the naive GAN inversion,
a more geometry-aware architecture such as 3D convolution used in cost volume based reconstruction methods~\misscite would likely to further improve the reconstruction performance on the novel views.

training side:
currently we need an extra 2D alignment module to assist the editing though lite, still introduces extra computational cost.
In the future work, we aim to find ways to remove this module without sacrificing the reconstruction ability,
and propose an end-to-end training strategy.

Overall,
we believe this work opens a new line of research direction and could serve as a guidance for future works beyond 3D GAN inversion, 
also few-shot 3D reconstructions and 3D-aware learning from 2D images, etc. 

\yslan{contribute: the merits of both priors.}

\yslan{out method could be easily extended to multi-view input.}


and takes a step towards expected 3D GAN inversion.


\heading{Limitations}
disadvantages:
slow sampling.

==> tables/3d_reconstruction_slam3r.tex <==
\begin{table*}[t]
  \centering
  \caption{\textbf{3D Reconstruction Comparison on 7-Scenes~\cite{Shotton_2013_CVPR}.} 
Here, we also include the comparison with recent work SLAM3R~\cite{slam3r}. While it runs at a higher frame rate, its performance is inferior. Note that we use SLAM3R$^*$ since the quantitative benchmark and FPS is evaluated on the $224\times224$ resolution, while all other methods are evaluated at $512\times384$ resolution.}
  \footnotesize
  \setlength{\tabcolsep}{0.3em}
  \begin{tabularx}{\textwidth}{>{\centering\arraybackslash}m{2.6cm} >{\centering\arraybackslash}m{0.9cm} >{\centering\arraybackslash}m{0.9cm} >{\centering\arraybackslash}X >{\centering\arraybackslash}X >{\centering\arraybackslash}X >{\centering\arraybackslash}X >{\centering\arraybackslash}X >{\centering\arraybackslash}X >{\centering\arraybackslash}m{0.9cm}}
    \toprule
    \multirow{3}{*}{\textbf{Method}} & \multirow{3}{*}{\textbf{Optim.}} & \multirow{3}{*}{\textbf{Onl.}} 
    & \multicolumn{2}{c}{{Acc}$\downarrow$} & \multicolumn{2}{c}{{Comp}$\downarrow$} & \multicolumn{2}{c}{{NC}$\uparrow$} 
    & \multirow{3}{*}{\textbf{FPS}} \\
    \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
     & & & Mean & Med. & Mean & Med. & Mean & Med. & \\
    % \midrule
    % VGG-T\footnotemark[1]~\cite{wang2025vggt} & & \checkmark
    %   & 0.087 & 0.039 & 0.091 & 0.039 & 0.787 & 0.890 & 12.0 \\
    \midrule
    DUSt3R-GA~\cite{wang2024dust3r} & \checkmark &
      & \underline{0.146} & \underline{0.077} & 0.181 & {0.067} & \bf 0.736 & \bf 0.839 & 0.68 \\
    MASt3R-GA~\cite{mast3r_arxiv24} & \checkmark &
      & 0.185 & 0.081 & {0.180} & 0.069 & 0.701 & 0.792 & 0.34 \\
    \monster{}-GA~\cite{zhang2024monst3r} & \checkmark &
      & 0.248 & 0.185 & 0.266 & 0.167 & 0.672 & 0.759 & 0.39 \\
    Spann3R~\cite{wang2024spann3r} & & \checkmark
      & 0.298 & 0.226 & 0.205 & 0.112 & 0.650 & 0.730 & 12.97 \\
    Fast3R~\cite{Yang_2025_Fast3R} & & \checkmark
      & 0.164 & 0.108 & 0.163 & 0.080 & 0.686 & 0.775 & \underline{30.92} \\
    SLAM3R$^*$~\cite{slam3r} & & \checkmark
      & 0.287 & 0.155 & 0.226 & 0.066 & 0.644 & 0.720 &  \bf 38.40 \\
    CUT3R~\cite{wang2025cut3r} & & \checkmark
      & \bf 0.126 & \bf 0.047 & \bf 0.154 & \bf 0.031 & \underline{0.727} & \underline{0.834} & 17.00 \\
    \nickname{} & & \checkmark
      & 0.148 &  \underline{0.077} &  \underline{0.177} &  \underline{0.058} & {0.700} & {0.801} & {26.40} \\
    \bottomrule
  \end{tabularx}
  \label{tab:3d_recon_withslam3r}
  \vspace{-3mm}
\end{table*}

% \begin{table*}[t]
%   \centering
%   \footnotesize
%   \setlength{\tabcolsep}{0.3em}
%   \begin{tabularx}{\textwidth}{l c c >{\centering\arraybackslash}X >{\centering\arraybackslash}X >{\centering\arraybackslash}X >{\centering\arraybackslash}X >{\centering\arraybackslash}X >{\centering\arraybackslash}X >{\centering\arraybackslash}X}
%     \toprule
%     & & & \multicolumn{6}{c}{\textbf{7 Scenes~\cite{Shotton_2013_CVPR}}} & \\
%     \cmidrule(lr){4-9}
%     & & & \multicolumn{2}{c}{{Acc}$\downarrow$} & \multicolumn{2}{c}{{Comp}$\downarrow$} & \multicolumn{2}{c}{{NC}$\uparrow$} & \textbf{FPS} \\
%     \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
%     \textbf{Method} & \textbf{Optim.} & \textbf{Onl.} & Mean & Med. & Mean & Med. & Mean & Med. & \\
%     \midrule
%     DUSt3R-GA~\cite{wang2024dust3r} & \checkmark &
%       & \underline{0.146} & \underline{0.077} & 0.181 & {0.067} & \bf 0.736 & \bf 0.839 & 0.68 \\
%     MASt3R-GA~\cite{mast3r_arxiv24} & \checkmark &
%       & 0.185 & 0.081 & {0.180} & 0.069 & 0.701 & 0.792 & 0.34 \\
%     \monster{}-GA~\cite{zhang2024monst3r} & \checkmark &
%       & 0.248 & 0.185 & 0.266 & 0.167 & 0.672 & 0.759 & 0.39 \\
%     Spann3R~\cite{wang2024spann3r} & & \checkmark
%       & 0.298 & 0.226 & 0.205 & 0.112 & 0.650 & 0.730 & 12.97 \\
%     Fast3R~\cite{Yang_2025_Fast3R} & & \checkmark
%       & 0.164 & 0.108 & 0.163 & 0.080 & 0.686 & 0.775 & \bf 30.92 \\
%     CUT3R~\cite{wang2025cut3r} & & \checkmark
%       & \bf 0.126 & \bf 0.047 & \bf 0.154 & \bf 0.031 & \underline{0.727} & \underline{0.834} & 17.00 \\
%     \nickname{} & & \checkmark
%       & 0.148 &  \underline{0.077} &  \underline{0.177} &  \underline{0.058} & {0.700} & {0.801} & \underline{26.4} \\
%     \midrule
%     VGG-T~\cite{wang2025vggt} & & \checkmark
%       & 0.087 & 0.039 & 0.091 & 0.039 & 0.787 & 0.890 & 12.0 \\
%     \bottomrule
%   \end{tabularx}
%   \caption{\textbf{3D reconstruction comparison on 7-Scenes~\cite{Shotton_2013_CVPR}.} 
% Despite operating in an online setting, our method delivers competitive performance—matching or even exceeding that of offline methods that leverage global alignment.  }
%   \label{tab:3d_recon}
% \end{table*}
